Modifying Memories in Transformer Models

Large Transformer models have achieved impressive performance in many natural language tasks. In particular, Transformer based language models have been shown to have great capabilities in encoding factual knowledge in their vast amount of parameters. While the tasks of improving the memorization and generalization of Transformers have been widely studied, it is not well known how to make transformers forget specific old facts and memorize new ones. In this paper, we propose a new task of \emph{explicitly modifying specific factual knowledge in Transformer models while ensuring the model performance does not degrade on the unmodified facts}. This task is useful in many scenarios, such as updating stale knowledge, protecting privacy, and eliminating unintended biases stored in the models. We benchmarked several approaches that provide natural baseline performances on this task. This leads to the discovery of key components of a Transformer model that are especially effective for knowledge modifications. The work also provides insights into the role that different training phases (such as pretraining and fine-tuning) play towards memorization and knowledge modification.

==> memorization.tex <==
\section{Memorization in Transformers}
\label{sec:memorization}
Generalization is important for implicit memorization. 
Require understanding of the semantics to generalize well. 


==> modification.tex <==
\section{Modifying facts while preserving generalization}
\label{sec:modification}
Our goal is to explore ways to modify memorized knowledge of the network while preserving its accuracy on unmodified facts.
In this way, we study the trade-off between memorizing certain new facts and preserving generalization on unmodified data. 
This also corresponds to the practical setting, where a user hopes to modify the response of the model on certain questions but also preserve the performance of the model on other questions.

In practice, the size of the training set is typically large. 
For efficient adaptation to modified facts, we focus on the setting of fine-tuning only on the training data corresponding to the modified examples. 
However, fine-tuning only on the small subset will undesirably cause overfitting, resulting in a significant drop in the accuracy on unmodified data. \zc{add results}
Therefore, we need to enforce a constraint on the increment of loss on the unmodified facts.
We formulate the task as
\begin{equation}
\begin{split}
\min_{\theta} & \frac{1}{|\gS'|}\sum_{i\in \gS'} L(x_i;\theta), \\
s.t.~& \frac{1}{|\gS|}\sum_{j\in \gS} L(x_j;\theta_0) - L(x_j;\theta) \le \delta.   \\
\end{split}
\end{equation}
Here $\gS$ is the set of all training samples, and $\gS'$ is the set of modified training samples. 
$\theta_0$ is the model parameters before fine-tuning on the modified facts. 
By default, $\theta_0$ was obtained by fine-tuning on the supporting evidences of the TREx dataset. 
Initializing from different parameters will result in different performances for the modification task. 

Enforcing the constraint on the whole training set is expensive. 
We need to find efficient proxies to reduce the cost of enforcing such constraints. 
One of the simplest proxies is to enforce a distance constraint between $\theta_0$ and $\theta$, since the function should not change too much when there are only slight changes to the parameters.
Specifically, we solve the following constrainted optimization in practice
\begin{equation}
\begin{split}
\min_{\theta} & \frac{1}{|\gS'|}\sum_{i\in \gS'} L(x_i;\theta), \\
s.t.~& \lVert \theta - \theta_0 \rVert \le \delta.   \\
\end{split}
\end{equation}
Empirically, we found using an $\ell_\infty$ norm constraint gives more stable results than $\ell_2$ norm, so we use $\ell_\infty$ norm by default. 

\subsection{Roles of Different Transformer Blocks}
When the number of training samples is small, the model tends to overfit. Such overfitting can be alleviated by controlling the number of learnable parameters, but which perparameters to train remains to be studied. \zc{Pending: experiments for fine-tuning the whole model on different number of modified samples. }
Intuitively, to modify the prediction of the model, we should fine-tune its classification head, and we do this by default. \zc{TODO: adding experiments to show this does not hurt. }
We found modifying the initial and final layers of the transformer results in better adaptation to modified facts and better preservation of performance on unmodified facts. 
This is partially consistent with the findings of~\cite{houlsby2019adaptor}, which demonstrated that fine-tuning some of the top layers of the bert\_base model are the best for certain tasks, except that we are also considering the model's performance on the hold-out unmodified facts, and found initial layers sometimes give better results for some models. 
\cite{zhang2019layerequal} also observed there exist some ambient layers in convolutional neural networks that do no affect the performance even if these layers are set to random initializations.
However, when fine-tuning on the whole TREx dataset, fine-tuning the whole network achieves better test results than fine-tuning one single layer. 
We give a formal defintion for this setting as 
\begin{equation}
\begin{split}
\min_{\theta^{(\gB)}} & \frac{1}{|\gS'|}\sum_{i\in \gS'} L(x_i;\theta), \\
s.t.~& \lVert \theta^{(\gB)} - \theta^{(\gB)}_0 \rVert \le \delta,   \\
\end{split}
\end{equation}
where $\gB$ is a set of indices and $\theta^{(\gB)}$ is a subset of the parameters, typically chosen as one or some of the transformer blocks. 

\paragraph{Criterion for selecting the best result.} 
The best model should achieve high accuracy on both the modified facts and the unmodified facts. 
For the interest of this problem, the accuracy on modified facts is more important. 
Therefore, we use the sum of the accuracy on modified and unmodified testing examples as the criterion, defined as
\begin{equation}
    \gA = \frac{1}{|\gS'_t|}\sum_{(x,y')\in \gS'_t} \indicator\{ x = y' \} + \frac{1}{|\gS_t \setminus \gS'_t|}\sum_{(x,y)\in \gS_t \setminus \gS'_t} \indicator\{ x = y \} 
\end{equation}
where $\gS_t$ is the full unmodified test set, and $\gS_t'$ is the modified subset of $\gS_t$. 



TODO: connect to previous visualization works 

\subsection{Modifying the Facts in Memory Networks}
Fact as Experts (FaE) incorporates 

\subsection{Effect of Fine-tuning on the Question Domain}
\begin{figure}
% \vspace{-2em}
\begin{center}
    \includegraphics[width=0.48\textwidth]{figures/compare_ftwhole_ftlayer.pdf}
\end{center}
\caption{\small The effect of fine-tuning the whole network on the QA domain.}
\label{fig:finetune_whole}
\end{figure}
\zc{Emphasize the importance of fine-tuning the whole network on the supporting sentences.}
\cite{neyshabur2020transfer} showed that pretrained models stays closer to the initialization than randomly initialized models after trained on a new domain. 
This indicates that pretraining enables the model to adapt to new tasks with milder change in its parameters. 
Similarly, in our setting, if the model has been fine-tuned as a whole on the QA domain, the model achieves better loss-gain curves than starting from a model that has only one transformer block fine-tuned on the QA domain, as shown in Figure~\ref{fig:finetune_whole}. 
\zc{maybe add comparisons with models that hasn't been fine-tuned at all. But these models have low accuracy on unmodified QAs anyway. }
This also demonstrates the importance of the hierarchical structure of BERT. \zc{relate to the discussions in \cite{neyshabur2020transfer}}

\subsection{Encoding Knowledge with Wide Transformers}
TODO: connect to previous works on adapters adding additional layers to different transformer blocks

Realm: Retrieval-augmented language model pre-training
ENRIE

\subsection{Experimental Setups}
Fine-tuning the model on TREx: tried learning rates from $\{5e-5, 8e-5, 1e-4\}$, epochs from 5 to 12.
We control the accuracy of the models on TREx to be roughly the same. 

\paragraph{Loss-gain curves}
\begin{figure}
% \vspace{-2em}
\begin{center}
    \includegraphics[width=0.5\textwidth]{figures/compare_l2_linf.pdf}
\end{center}
\caption{\small Comparing $\ell_2$ and $\ell_\infty$ constraints.}
\label{fig:transformer_blocks}
\end{figure}
To evaluate the performance of a certain approach in modifying the factual knowledge, we plot the loss-gain tradeoff as we loose the constraints. 
The loss is defined as the absolute decrease of accuracy on unmodified facts after the model is fine-tuned on the modified training samples. 
The gain is defined as the absolute increase in accuracy on modified facts for the same model. \zc{TODO: add notations for these concepts.}
Choice of the norms: as shown in Figure~\ref{fig:transformer_blocks}, there are no significant differences between using $\ell_2$ or $\ell_\infty$ norm as the constraints, in terms of the optimal tradeoff they can achieve. 
However, we find less back-and-forth in the the curves using the $\ell_\infty$ constraints.
This indicates it is easier for the model to find good minima under $\ell_\infty$ constraints. 
To serve the purpose of this paper, we choose $\ell_\infty$ constraints when plotting the loss-gain curves. 

\begin{figure}
% \vspace{-2em}
\begin{center}
    \includegraphics[width=0.45\textwidth]{figures/direct_finetune_addedonly.pdf}
    \includegraphics[width=0.45\textwidth]{figures/direct_finetune_wholeblock.pdf}

    \includegraphics[width=0.45\textwidth]{figures/trexft_addonly.pdf}
    \includegraphics[width=0.45\textwidth]{figures/trexft_wholeblock.pdf}
    
    \includegraphics[width=0.45\textwidth]{figures/bertpt_trexft_addonly.pdf}
    \includegraphics[width=0.45\textwidth]{figures/bertpt_trexft_wholeblock.pdf}
\end{center}
\caption{\small AddOnly: only training added weights on modified facts. FT: the model has been fine-tuned on the TREx training set. PT: the model has been pretrained on Wikipedia and BookCorpus.  \zc{TODO: add the curves for fine-tuning each single layer without additional weights. Evaluate under $\ell_2$ norms.}}
\label{fig:transformer_blocks}
\end{figure}
Assumption: all the parameters are useful for memorization. 

\paragraph{Fine-tuning whole block vs. only additional weights} 
We hope by only fine-tuning the additional weights in the wide layers, we can store the modified facts into the additional weights and minimize their influence on the memorized facts. 
However, the results show that fine-tuning only the additional weights does not outperform fine-tuning the whole transformer block. 
We can at least conclude that other weights in the transformer block are equally important for memorizing new facts.

\paragraph{Lottery Ticket?}
Can we progressively prune the network trained on TREx to revel which weights are more important for generalization?

\paragraph{Effect of pretraining}
Pretraining the added weights does not seem to help. It does not boost the performance of additional layers to the same level as fine-tuning the whole network. 
The modification results is not as good. 

\paragraph{Effect of adding more parameters}
The effect of adding more parameters seems marginal. Should we instead prune the parameters, or observing the results of distillation models?

\paragraph{Training various blocks?}
Layer 11 is consistently better in all settings

\paragraph{Effect of problem difficulty}
\begin{figure}
% \vspace{-2em}
\begin{center}
    \includegraphics[width=0.45\textwidth]{figures/num_facts/trex_nfacts_10epochs_layer0.pdf}
    % \includegraphics[width=0.45\textwidth]{figures/num_facts/trex_nfacts_10epochs_layer5.pdf}
    \includegraphics[width=0.45\textwidth]{figures/num_facts/trex_nfacts_10epochs_layer11.pdf}
\end{center}
\caption{\small Loss-gain curves under different numbers of modified facts.}
\label{fig:transformer_blocks}
\end{figure}
Our ideal goal is to obtain perfect accuracy on the modified facts, since they are usually more important to the users. 
When the model does not have perfect generalization, in the extreme case where we modify all the facts, the generalization on the modified facts can be at most the same as on the unmodified samples before modification. 
By contrast, if we only modify the model's predictions for one fact, then it is easier to preserve the the model's prediction on other facts. 
Intuitively, the frequency of the modified answer should also affect the loss-gain tradeoff. \zc{TODO: add more explanations.}
To quantify the difficulty of the task, we plot the loss-grain curves at different number of modified facts, and the different frequencies of the answer to be modified into. 
The results are shown in Figure~\ref{fig:transformer_blocks}. 
As expected, it becomes more difficult for the model to achieve high accuracies on more modified facts. 
The difference between using high frequency and similar frequency answers are not always consistent, but when modifying the answers into rare answers, the results become much more different, typically bad. 
This indicates the model has not learned to generalize well on rare facts. \zc{More here?}


\subsection{Preserving knowledge with few unmodified samples}
In each iteration, we should use both the modified samples and the unmodified samples, so that the model can fit to the modified facts well. 
We need to evaluate the number of additional training samples used, and the ratio of the batch sizes. 

\subsection{Theoretical insights?}
Improved generalization bound under constraints? There is a paper on that, but the proof seems problematic. \ankit{Is this paper available on arXiv?}\zc{Yes: https://arxiv.org/pdf/2002.08253.pdf. But I think their proof for Theorem 2 is problematic. They missed the Rademacher complexity term on the input data when iteratively expanding inequality (iii). Their proof technique should only be able to achieve a looser bound than their Lemma 2 and does not show why constraint helps.}

Capacity vs generalization? 

Parameter-counting based generalization bound improves when fewer layers of the network is trained~\citep{zhang2019layerequal}. Can we also relate this to the results in~\citep{feldman2020longtail}?

Observations: 1) fine-tuning the whole network on the same domain as the facts to be modified, followed by fine-tuning some of the layers on the modified facts, gives better tradeoffs than fine-tuning a single block on the same domain in the first step. 2) Initial and Final blocks are better for modification task.

Hypothesis: 1) Higher layers generalizing better is consistent with results from~\cite{neyshabur2020transfer}. 2) The weights of pretrained models does not change much after fine-tuned on another task~\cite{neyshabur2020transfer}. Therefore, fine-tuned models can fit the modified data better without much influence on unmodified samples. 3) The weight change of wider models is smaller to overfit the data. This somehow contradicts with the fact that training one block is better than training the whole model. Need to double check the details of~\cite{neyshabur2019towards}.


==> tables.tex <==
\begin{table*}[!t]
%\begin{wraptable}{r}{7.0cm}
   \footnotesize
    \centering
    \setlength{\tabcolsep}{3.5pt}   
    %
    \scalebox{0.87}{
    \begin{tabular}{ccccc|ccc|ccc}%{lllll|lll|lll}
    \toprule
    \multicolumn{2}{c}{} &
    \multicolumn{3}{c}{{\sc AmazonCat-13k}}   &
    \multicolumn{3}{c}{{\sc WikiLSHTC-325k}} &
    \multicolumn{3}{c}{{\sc AmazonCat-670k}} \\
    \cmidrule{3-5} \cmidrule{6-8} \cmidrule{9-11}
        {\bf Metric} &{\bf Method}   & \spa & \spb  & \full & \spa & \spb & \full& \spa & \spb & \full\\
        \toprule 
\multirow{4}{*}{{\rm recall}@1} & Top-$256$ & 0.3982 & 0.1075 & 0.1753 & 0.2482 & 0.1603 & 0.1681 & \best{0.0973} & 0.0708 & \best{0.0774} \\
& Top-$512$ & 0.4034 & \best{0.1130} & 0.1765 & 0.2499 & 0.1636 & 0.1696 & 0.0972 & 0.0705 & 0.0768 \\
& Top-$1024$ & \best{0.4016} & 0.1109 & \best{0.1788} & \best{0.2504} & 0.1681 & \best{0.1708} & 0.0948 & \best{0.0732} & 0.0771 \\
&  All $2048$ (SNM)  & 0.3836 & 0.1031 & 0.1785 & 0.2299 & \best{0.1722} & 0.1699 & 0.0825 & 0.0698 & 0.0745 \\
\cmidrule{2-11}
\multirow{4}{*}{{\rm recall}@5} & Top-$256$ & 0.8126 & 0.5295 & 0.5873 & 0.5636 & 0.3960 & 0.4116 & 0.4224 & 0.2892 & \best{0.3192} \\
& Top-$512$ & 0.8245 & 0.5380 & 0.5938 & \best{0.5714} & 0.4058 & 0.4187 & \best{0.4228} & 0.2903 & 0.3169 \\
& Top-$1024$ & \best{0.8441} & \best{0.5516} & 0.6065 & 0.5673 & \best{0.4147} & \best{0.4237} & 0.4163 & \best{0.2989} & \best{0.3192} \\
&  All $2048$ (SNM)  & 0.8318 & 0.5454 & \best{0.6113} & 0.5126 & 0.3984 & 0.4021 & 0.3775 & 0.2910 & 0.3084 \\
\cmidrule{2-11}
\multirow{4}{*}{{\rm recall}@10} & Top-$256$ & 0.9113 & 0.6964 & 0.7324 & 0.6757 & 0.4962 & 0.5073 & 0.5611 & 0.3947 & 0.4291 \\
& Top-$512$ & 0.9157 & 0.7084 & 0.7397 & 0.6871 & 0.5103 & 0.5189 & \best{0.5665} & 0.3998 & 0.4305 \\
& Top-$1024$ & \best{0.9260} & \best{0.7195} & 0.7485 & \best{0.6875} & \best{0.5238} & \best{0.5291} & 0.5651 & \best{0.4138} & \best{0.4369} \\
&  All $2048$ (SNM)  & 0.9056 & 0.7083 & \best{0.7416} & 0.6362 & 0.5052 & 0.5091 & 0.5274 & 0.4100 & 0.4307 \\
\cmidrule{2-11}
 \multirow{4}{*}{{\rm recall}@25} & Top-$256$ & 0.9708 & 0.8618 & 0.8635 & 0.7750 & 0.6063 & 0.6064 & 0.6426 & 0.4776 & 0.5050 \\
& Top-$512$ & \best{0.9710} & 0.8657 & 0.8664 & 0.7885 & 0.6247 & 0.6232 & 0.6534 & 0.4884 & 0.5125 \\
& Top-$1024$ & 0.9700 & \best{0.8736} & \best{0.8685} & \best{0.7925} & \best{0.6423} & \best{0.6392} & \best{0.6598} & 0.5111 & 0.5272 \\
&  All $2048$ (SNM)  & 0.9517 & 0.8459 & 0.8513 & 0.7597 & 0.6285 & 0.6289 & 0.6372 & \best{0.5146} & \best{0.5334} \\

        \bottomrule
    \end{tabular}
    }
    \caption{Test set recall on \amazonsmall,~\wikilshtc, and~\amazonmedium, where the evaluation focuses on two subpopulations (\spa~and~\spb) based on label popularity. We assess \SSNM{} for varying values of $\kExample$, on a minibatch size of $\MinibatchSize = 2048$. Note that SNM corresponds to choosing $\kExample = 2048$. During each optimization step, we select the $\kLabel = 64$ ($\kLabel=1$) hardest negative labels from a set of $\bar{\NumLabels} = 4096$ randomly sampled negative labels for \amazonsmall~(\wikilshtc~and~\amazonmedium). {In almost all cases, the best performance is achieved by choosing $\kExample < 2048$}, {thus validating the efficacy of \SSNM{}}.
    }
    \label{tbl:results-multilabel}
    \vspace{-\baselineskip}
%\end{wraptable}
\end{table*}



\begin{table*}[h]
%\begin{wraptable}{r}{7.0cm}
  \vspace{-1mm}
   \footnotesize
    \centering
    \setlength{\tabcolsep}{4pt}   
    %
    \scalebox{0.85}{
    \begin{tabular}{ccccc|cccc|cccc}%{lllll|llll|llll}
    \toprule
    \multicolumn{1}{l}{} &
    \multicolumn{4}{c}{\amazonsmall}   &
    \multicolumn{4}{c}{\wikilshtc} &
    \multicolumn{4}{c}{\amazonmedium} \\
    \cmidrule{2-5} \cmidrule{6-9} \cmidrule{10-13}
        {\bf Method}   & {\bf P@1} & {\bf P@3}& {\bf P@5} & {\bf P@10} & {\bf P@1} & {\bf P@3}& {\bf P@5} & {\bf P@10} & {\bf P@1} & {\bf P@3}& {\bf P@5} & {\bf P@10}\\
        \toprule 
Top-$256$ & 0.8965 & 0.7397 & 0.6004 & 0.3746 & 0.5456 & 0.3764 & 0.2884 & 0.1842 & 0.4036 & 0.3644 & 0.3330 & 0.2236   \\
Top-$512$ & 0.9028 & 0.7481 & 0.6072 & 0.3786 & 0.5531 & 0.3838 & 0.2955 & 0.1897 & 0.4021 & 0.3641 & 0.3329 & 0.2253   \\
Top-$1024$ & 0.9132 & 0.7639 & 0.6198 & \best{0.3828} & 0.5608 & \best{0.3897} & \best{0.3010} & \best{0.1945} & \best{0.4055} & \best{0.3677} & \best{0.3350} & \best{0.2287}   \\
All $2048$ (SNM) & \best{0.9155} & \best{0.7717} & \best{0.6247} & {0.3795} & \best{0.5610} & 0.3751 & 0.2885 & 0.1883 & 0.3927 & 0.3571 & 0.3237 & 0.2253   \\
        \bottomrule
    \end{tabular}
    }
    \caption{Performance of \SSNM{} on \amazonsmall, \wikilshtc, and \amazonmedium, as measured by {\rm Precision@}$r$ or P@$r$. Note that \SSNM{} is competitive with SNM, i.e., using all examples in the minibatch of size $2048$. These results show that, while we focus on evaluating the retrieval performance of our proposed on different sub-populations (cf.~Table~\ref{tbl:results-multilabel}), it provides competitive or better performance in terms of the widely reported Precision metric on the original test sets.}
    \label{tbl:precision-extreme}
    \vspace{-\baselineskip}
%\end{wraptable}
\end{table*}




==> tables/bert_base_layerwise.tex <==
\begin{table}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ l|c|c|c|c|c|c|c|c|c|c|c|c } 
\hline
Layers & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11\\
\hline
$\delta$ & 0.005 & 0.01 & 0.01 & 0.005 & 0.005 & 0.005 & 0.005 & 0.005 & 0.01 & 0.005 & 0.002 & 0.005\\
\hline
$\mathfrak{A}_{\gF\setminus \gS}$ & 43.80 & 39.04 & 40.30 & 43.87 & 37.76 & 40.52 & 39.96 & 41.70 & 33.95 & 36.21 & 44.07 & 42.17\\
\hline
$\mathfrak{A}_{ \gM}$ & 78.12 & 75.00 & 78.12 & 68.75 & 78.12 & 68.75 & 71.88 & 68.75 & 68.75 & 71.88 & 71.88 & 78.12\\
\hline
\end{tabular}
}
\caption{Best results for fine-tuning each Transformer block of bert\_base on modified facts under various $\ell_\infty$ constraints. \zc{These }}
\end{table}

==> tables/bert_large_layerwise.tex <==
\begin{table}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ l|c|c|c|c|c|c|c|c|c|c|c|c } 
\hline
Layers & 0 & 2 & 4 & 6 & 8 & 10 & 12 & 14 & 16 & 18 & 20 & 22\\
\hline
$\delta$ & 0.004 & 0.008 & 0.008 & 0.008 & 0.008 & 0.008 & 0.008 & 0.004 & 0.016 & 0.008 & 0.004 & 0.008\\
\hline
$\mathfrak{A}_{\gF\setminus \gS}$ & 48.51 & 47.45 & 44.74 & 43.45 & 45.78 & 45.11 & 44.81 & 42.22 & 30.40 & 41.75 & 41.88 & 41.95\\
\hline
$\mathfrak{A}_{ \gM}$ & 71.88 & 78.12 & 75.00 & 75.00 & 75.00 & 68.75 & 71.88 & 62.50 & 68.75 & 59.38 & 68.75 & 78.12\\
\hline
\end{tabular}
}
% \caption{}
\end{table}

==> tables/permutation.tex <==
\begin{table}[htbp!]
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|c|c|c|c|c|c}
\hline
Dataset       & \multicolumn{3}{c|}{$|\gM|=32$}           & \multicolumn{3}{c}{$|\gM|=32$, permuted}         \\ \hline
Layer         & 0            & 5            & 11           & 0            & 5            & 11           \\ \hline
$\mathfrak{A}_{RI}$    & 13.75 (3.49) & 16.25 (1.05) & 16.25 (1.85) & 15.00 (1.05) & 15.00 (1.63) & 18.12 (0.56)  \\ \hline
$\mathfrak{A}_{PT}$    & 75.00 (3.19) & 66.25 (2.40) & 67.50 (1.12) & 71.88 (1.98) & 56.88 (3.35) & 56.88 (2.40)  \\ \hline
$\mathfrak{A}_{PT+FT}$ & 77.50 (2.40) & 77.50 (1.37) & 82.50 (2.27) & 75.00 (2.50) & 65.00 (2.05) & 63.75 (2.27) \\ \hline
$\mathfrak{A}_{PT+FTP}$ & 71.25 (2.71) & 71.88 (1.98) & 79.38 (2.88) & 72.50 (3.47) & 70.00 (1.12) & 76.88 (2.27)\\ \hline
\end{tabular}
}
\caption{Comparing the test accuracy on the standard and permuted datasets after trained on the corresponding training sets of 32 modified facts for a randomly initialized bert\_base ($\gA_{RI}$ ), a pretrained bert\_base ($\gA_{PT}$), a pretrained bert\_base fine-tuned on the TREx dataset ($\gA_{PT+FT}$), and the same pretrained bert\_base fine-tuned on the permuted TREx dataset ($\gA_{PT+FTP}$). For "$|\gM|=32$, permuted", we apply a fixed random permutation to $\gD_{M}$. We compute the mean and standard error of the accuracy over 5 runs with different random seeds. }
\label{tab:perm}
\end{table}

==> tables/permutation_128.tex <==
\begin{table}[htbp!]
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|c|c|c|c|c|c}
\hline
Dataset       & \multicolumn{3}{c|}{$\gS'_{128}$}           & \multicolumn{3}{c}{$\gS'_{128,p}$}         \\ \hline
Layer         & 0            & 5            & 11           & 0            & 5            & 11           \\ \hline
$\mathfrak{A}_{RI}$    & 17.97 (1.15) & 13.91 (0.81) & 11.88 (0.46) & 13.28 (1.06) & 12.66 (0.87) & 8.91 (0.36)  \\ \hline
$\mathfrak{A}_{PT}$    & 78.91 (0.38) & 75.47 (1.41) & 64.38 (1.51) & 81.25 (0.77) & 54.69 (2.01) & 38.75 (0.87)  \\ \hline
$\mathfrak{A}_{PT+FT}$ & 80.00 (0.81) & 75.31 (1.05) & 82.03 (0.99) & 72.34 (0.84) & 67.03 (1.54) & 58.75 (0.68) \\ \hline
\end{tabular}
}
\label{tab:perm128}
\caption{Same setting as Table~\ref{tab:perm}, except for modifying 128 facts. }
\end{table}

==> tables/permutation_2048.tex <==
\begin{table}[htbp!]\label{tab:perm2048}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|c|c|c|c|c|c}
\hline
Dataset       & \multicolumn{3}{c|}{$\gS'_{2048}$}           & \multicolumn{3}{c}{$\gS'_{2048,p}$}         \\ \hline
Layer         & 0            & 5            & 11           & 0            & 5            & 11           \\ \hline
$\mathfrak{A}_{RI}$    & 19.14 (0.34) & 15.17 (0.79) & \zc{6.10 (0.69)} & 19.53 (0.86) & 16.83 (0.74) & 9.52 (0.24)  \\ \hline
$\mathfrak{A}_{PT}$    & 52.62 (0.68) & 59.68 (0.59) & 49.38 (0.32) & 53.86 (0.09) & 38.95 (0.30) & 24.11 (0.11)  \\ \hline
$\mathfrak{A}_{PT+FT}$ & 48.51 (0.74) & 70.09 (0.34) & 57.67 (1.84) & 51.75 (0.63) & 38.49 (0.61) & 26.16 (0.14)\\ \hline
\end{tabular}
}
\caption{Same setting as Table~\ref{tab:perm}, except for modifying 2048 facts. }
\end{table}

==> tables/permutation_512.tex <==
\begin{table}[htbp!]\label{tab:perm512}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|c|c|c|c|c|c}
\hline
Dataset       & \multicolumn{3}{c|}{$\gS'_{512}$}           & \multicolumn{3}{c}{$\gS'_{512,p}$}         \\ \hline
Layer         & 0            & 5            & 11           & 0            & 5            & 11           \\ \hline
$\mathfrak{A}_{RI}$    & 14.80 (0.83) & 12.97 (0.52) & 7.54 (0.25) & 14.37 (0.62) & 12.50 (0.77) & 8.09 (0.72)  \\ \hline
$\mathfrak{A}_{PT}$    & 70.86 (0.34) & 78.63 (0.84) & 64.38 (2.23) & 71.13 (0.34) & 53.12 (0.26) & 37.15 (0.53)  \\ \hline
$\mathfrak{A}_{PT+FT}$ & 68.36 (0.73) & 76.21 (0.44) & 73.83 (1.08) & 59.57 (0.86) & 53.59 (7.58) & 47.19 (0.73) \\ \hline
\end{tabular}
}
\caption{Same setting as Table~\ref{tab:perm}, except for modifying 512 facts.}
\end{table}

==> tables/transfer_vs_modify.tex <==
\begin{table}[htbp!]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|c|c|c|c|c|c}
\hline
Dataset                       & \multicolumn{3}{c|}{$\gS'_{128}$}          & \multicolumn{3}{c}{$\gS'_{2048}$} \\ \hline
Layer                         & 0            & 5            & 11           & 0         & 5         & 11         \\ \hline
$\mathfrak{A}_{TL, \gS'}$              & 83.33 (1.06) & 77.08 (1.18) & 78.12 (0.97) & 47.35 (0.87) & 69.37 (0.37) &  56.52 (0.28)  \\ \hline
$\mathfrak{A}_{TL, \gS\setminus \gS'}$ & 2.89 (0.46)  & 19.44 (0.50) & 4.29 (0.33)  & 0.57 (0.04)  &  1.01 (0.07) & 0.65 (0.08)  \\ \hline
$\mathfrak{A}_{M, \gS'}$               & 80.00 (0.81) & 75.31 (1.05) & 82.03 (0.99) & 48.53 (0.75) & 70.17 (0.33) & 57.67 (1.84)  \\ \hline
$\mathfrak{A}_{M, \gS\setminus \gS'}$  & 4.40 (0.75)  & 18.64 (1.10) & 3.90 (0.36)  & 0.58 (0.03) & 1.13 (0.06) & 0.91 (0.06) \\ \hline
\end{tabular}
}
\caption{Comparing the test accuracy on modified facts for the transfer learning and the knowledge modification setting. Any $\mathfrak{A}$ with subscript $TL$ or $M$ is the accuracy achieved under the Transfer Learning or Modification setting. \zc{Results with 128 facts does not show modification causes more negative impact on the model's performance, not as expected. Waiting for the results with 2048 modifications. A good side of the current result is that TL either has higher accuracy on both $\gS'$ and $\gS\setminus \gS'$, or only has one of them worse than M.}}
\label{tab:tl_vs_m}
\end{table}
